3D non-LTE line formation of neutral carbon in the Sun

Carbon abundances in late-type stars are important in a variety of astrophysical contexts. However C i lines, one of the main abundance diagnostics, are sensitive to departures from local thermodynamic equilibrium (LTE). We present a model atom for non-LTE analyses of C i lines, that uses a new, physically-motivated recipe for the rates of neutral hydrogen impact excitation. We analyse C i lines in the solar spectrum, employing a three-dimensional (3D) hydrodynamic model solar atmosphere and 3D non-LTE radiative transfer. We find negative non-LTE abundance corrections for C i lines in the solar photosphere, in accordance with previous studies, reaching up to around 0.1 dex in the disk-integrated flux. We also present the first fully consistent 3D non-LTE solar carbon abundance determination: we infer log $\epsilon_{\text{C}}$ = $8.44\pm0.02$, in good agreement with the current standard value. Our models reproduce the observed solar centre-to-limb variations of various C i lines, without any adjustments to the rates of neutral hydrogen impact excitation, suggesting that the proposed recipe may be a solution to the long-standing problem of how to reliably model inelastic collisions with neutral hydrogen in late-type stellar atmospheres.

==> journals.tex <==

\def\memsai{Mem. Societa Astronomica Ital. }
\def\aj{AJ}
\def\actaa{Acta Astronomica}
\def\araa{ARA\&A}
\def\apj{ApJ}
\def\apjl{ApJ}
\def\apjs{ApJS}
\def\ao{Appl.~Opt.}
\def\apss{Ap&SS}
\def\aap{A\&A}
\def\aapr{A\&A Rev.}
\def\aaps{A\&AS}
\def\azh{Astronomicheskii Zhurnal}
\def\baas{BAAS}
\def\caa{Chinese Astronomy and Astrophysics}
\def\cjaa{Chinese Journal of Astronomy and Astrophysics}
\def\icarus{Icarus}
\def\jcap{Journal of Cosmology and Astroparticle Physics}
\def\jrasc{JRASC}
\def\memras{MmRAS}
\def\mnras{MNRAS}
\def\na{New Astronomy}
\def\nar{New Astronomy Review}
\def\pra{Phys.~Rev.~A}
\def\prb{Phys.~Rev.~B}
\def\prc{Phys.~Rev.~C}
\def\prd{Phys.~Rev.~D}
\def\pre{Phys.~Rev.~E}
\def\prl{Phys.~Rev.~Lett.}
\def\pasa{Publications of the Astron. Soc. of Australia}
\def\pasp{PASP}
\def\pasj{PASJ}
\def\rmxaa{Revista Mexicana de Astronomia y Astrofisica}
\def\qjras{QJRAS}
\def\skytel{S\&T}
\def\solphys{Sol.~Phys.}
\def\sovast{Soviet Astronomy}
\def\ssr{Space Sci.~Rev.}
\def\zap{Zeitschrift fuer Astrophysik}
\def\nat{Nature}
\def\iaucirc{IAU Circ.}
\def\aplett{Astrophys.~Lett.}
\def\apspr{Astrophys.~Space Phys.~Res.}
\def\bain{Bull.~Astron.~Inst.~Netherlands}
\def\fcp{Fund.~Cosmic Phys.}
\def\gca{Geochimica Cosmochimica Acta}
\def\grl{Geophysics Research Letters}
\def\jcp{Journal of Chemical Physics}
\def\jgr{Journal of Geophysics Research}
\def\jqsrt{Journal of Quantitiative Spectroscopy and Radiative Transfer}
\def\memsai{Mem. Societa Astronomica Ital.}
\def\nphysa{Nuclear Physics A}
\def\physrep{Physics Reports}
\def\physscr{Physica Scripta}
\def\planss{Planet.~Space Sci.}
\def\procspie{Proc.~SPIE}


